PhysAvatar: Learning the Physics of Dressed 3D Avatars from Visual Observations

Modeling and rendering photorealistic avatars is of crucial importance in many applications. Existing methods that build a 3D avatar from visual observations, however, struggle to reconstruct clothed humans. We introduce PhysAvatar, a novel framework that combines inverse rendering with inverse physics to automatically estimate the shape and appearance of a human from multi-view video data along with the physical parameters of the fabric of their clothes. For this purpose, we adopt a mesh-aligned 4D Gaussian technique for spatio-temporal mesh tracking as well as a physically based inverse renderer to estimate the intrinsic material properties. PhysAvatar integrates a physics simulator to estimate the physical parameters of the garments using gradient-based optimization in a principled manner. These novel capabilities enable PhysAvatar to create high-quality novel-view renderings of avatars dressed in loose-fitting clothes under motions and lighting conditions not seen in the training data. This marks a significant advancement towards modeling photorealistic digital humans using physically based inverse rendering with physics in the loop. Our project website is at: https://qingqing-zhao.github.io/PhysAvatar

==> figs/relighting.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/relighting.pdf}
    \vspace{5pt}
    \caption{Relighting results of our method.}
    \label{fig:application}
\end{figure}

==> figs/results_mixamo.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure/results_mixamo.pdf}
    \vspace{1pt}
    \caption{Our results on challenging motions from Mixamo~\cite{Mixamo}.}
    \label{fig:results_mixamo}
\end{figure}
